Attacking Perceptual Similarity Metrics

Perceptual similarity metrics have progressively become more correlated with human judgments on perceptual similarity; however, despite recent advances, the addition of an imperceptible distortion can still compromise these metrics. In our study, we systematically examine the robustness of these metrics to imperceptible adversarial perturbations. Following the two-alternative forced-choice experimental design with two distorted images and one reference image, we perturb the distorted image closer to the reference via an adversarial attack until the metric flips its judgment. We first show that all metrics in our study are susceptible to perturbations generated via common adversarial attacks such as FGSM, PGD, and the One-pixel attack. Next, we attack the widely adopted LPIPS metric using spatial-transformation-based adversarial perturbations (stAdv) in a white-box setting to craft adversarial examples that can effectively transfer to other similarity metrics in a black-box setting. We also combine the spatial attack stAdv with PGD ($\ell_\infty$-bounded) attack to increase transferability and use these adversarial examples to benchmark the robustness of both traditional and recently developed metrics. Our benchmark provides a good starting point for discussion and further research on the robustness of metrics to imperceptible adversarial perturbations.

==> algos/1pix.tex <==
\makeatletter
\newcommand{\removelatexerror}{\let\@latex@error\@gobble}
\makeatother
\begingroup
\removelatexerror
\begin{algorithm}[H]
\footnotesize
\KwInput{$I_0$, $I_1$, $I_{ref}$, trained LPIPS model $f$}
\KwOutput{x\_position, y\_position, r, g, b of the perturbation}
\SetKwFunction{FMain}{PerturbImage}
\SetKwProg{Fn}{Function}{:}{}
\Fn{\FMain{$I_{prey}$, $I_{ref}$, $s_{other}$, $T$}}{
    
    population\_size = len($T$) // Trial vector $T$ \\
    
    $I_{adv}$ = repeat($I_{prey}$, population\_size) // create batch \\
    
    factor = 0.1
    
    \For{i $\leftarrow$ 1 to population\_size}{
        // Apply perturbation to each $I^i_{adv}$ \\
        x\_position, y\_position, r, g, b = $T_i$ \\
        $I_{adv}$[i, 0, x\_position, y\_position] = (r/255 - 0.5)/factor \\
        $I_{adv}$[i, 1, x\_position, y\_position] = (g/255 - 0.5)/factor \\
        $I_{adv}$[i, 2, x\_position, y\_position] = (b/255 - 0.5)/factor \\
        $s^i_{adv} = f(I_{ref}, I_{adv})$ \\
        $s^i = 1 - (s_{adv}^i/(s_{adv}^i+s_{other}^i))$ // Fitness score \\
        // If score $s^i$ of $T_i$ is better than the score of $X_i$ \\ 
        // then $T_i$ replaces $X_i$ during differential evolution \\
    }
    \KwRet{$s$ // scores} \
    }{}{}
  \setcounter{AlgoLine}{0}
$s_0 = f(I_{ref}, I_0)$; $s_1 = f(I_{ref}, I_1)$; \\

// If $I_0$ is more similar to $I_{ref}$ then $rank$ is 0 else 1 \\
$rank = int(s_0 > s_1)$ // smaller $s_i$ $\equiv$ more similar \\

\lIf*{ $rank = 1$ } {
    $I_{prey}$ = $I_1$; $s_{other}$ = $s_0$;
} \\
\lElse*{
    $I_{prey}$ = $I_0$; $s_{other}$ = $s_1$;
}

successfull\_vector\_$X_i$ = differential\_evolution(func=PerturbImage, args=($I_{prey}$, $I_{ref}$, $s_{other}$)) \\
// The differential\_evolution algorithm optimizes population $X$  \\
// to find optimal $X_i^*$ (see Figure~\ref{fig:de}) \\

x\_position, y\_position, r, g, b = successfull\_vector\_$X_i$ \\

\Return{x\_position, y\_position, r, g, b}
\caption{One-pixel attack on LPIPS}
\label{algo:1pix}
\end{algorithm}
\endgroup
